Multi-Review Fusion-in-Context

Grounded text generation, encompassing tasks such as long-form question-answering and summarization, necessitates both content selection and content consolidation. Current end-to-end methods are difficult to control and interpret due to their opaqueness. Accordingly, recent works have proposed a modular approach, with separate components for each step. Specifically, we focus on the second subtask, of generating coherent text given pre-selected content in a multi-document setting. Concretely, we formalize Fusion-in-Context (FiC) as a standalone task, whose input consists of source texts with highlighted spans of targeted content. A model then needs to generate a coherent passage that includes all and only the target information. Our work includes the development of a curated dataset of 1000 instances in the reviews domain, alongside a novel evaluation framework for assessing the faithfulness and coverage of highlights, which strongly correlate to human judgment. Several baseline models exhibit promising outcomes and provide insightful analyses. This study lays the groundwork for further exploration of modular text generation in the multi-document setting, offering potential improvements in the quality and reliability of generated content. Our benchmark, FuseReviews, including the dataset, evaluation framework, and designated leaderboard, can be found at https://fusereviews.github.io/.

==> sections/deprecated/4_crowdsourcing_deprecated.tex <==
\input{tables/data_statistics}

\section{Data Construction}\label{sec:crowdsourcing}
Inspired by \citep{slobodkin-etal-2022-controlled}, We leverage existing multi-review summarization datasets to annotate a high-quality FiC dataset.
Recognizing that summaries are typically derived from a set of salient spans within the input texts, our annotation methodology seeks to 'reverse-engineer' this process. The goal is to identify the specific excerpts in the source reviews that contributed to the creation of a given summary.
This approach significantly streamlines the annotation process. Instead of the demanding task of generating a new text from highlighted spans, annotators focus on identifying relevant spans within reviews that correlate with a provided summary. This method effectively reduces both the complexity and the workload of the annotation task, facilitating a more efficient and focused data collection process.

For the dataset construction, we sample 220 distinct review-sets from the CocoTrip dataset \citep{iso22aclfindings}, a comparative opinion summarization dataset of hotels reviews, and 100 distinct review-sets from the FewSum dataset \citep{brazinskas2020few}, consisting of summaries of various businesses reviews. Each set comprises 8 reviews, and comes with up to 6 different reference summaries, averaging 3.13 summaries per set. This results in a total of 1000 unique summary-review set pairings (see \autoref{tab:dataset_statistics} for full statistics).\footnote{We use spaCy \cite{spacy2} for tokenization and sentence separation.}
Due to the task's complexity, we employ a \textit{controlled crowdsourcing} framework \citep{roit-etal-2020-controlled}, which includes structured stages of annotators recruitment and training, thereby ensuring the employment of a competent and reliable group of annotators for the dataset annotation.

\subsection{Annotation Process} \label{subsec:Annotation Process}
For the annotation of review spans corresponding to summary content, we adapt a web-based interface,\footnote{\url{https://github.com/lovodkin93/highlights-extract-app}} that is published on Amazon Mechanical Turk\footnote{\url{www.mturk.com}} and used by crowd-workers. Annotators are presented with summaries and corresponding reviews in a side-by-side format, tasked with highlighting review spans that relate to the summary content. To reduce cognitive load, each summary is displayed alongside individual reviews.
Annotators are instructed to align specific aspects of a business, such as room cleanliness, from the summary with the most relevant spans in the reviews.
This method entails creating alignments for each business characteristic mentioned in the summary.

We observed that focusing on one business characteristic at a time enhances the annotators' efficiency in identifying the relevant spans, particularly when a summary sentence includes descriptions scattered across different parts of the review.
Further, to facilitate the process, significant words in the reviews are emboldened if they share lemmas with words in the current summary sentence, utilizing spaCy \cite{spacy2} for lemmatization.
This approach allows annotators to quickly skim through reviews with minimal bias.
It is presumed that trained workers will not rely solely on same-lemma words for highlighting, as per the guidelines provided (see \S\ref{subsec:guidelines}).

Once a trained pool of workers is established (see \S\ref{subsec:Annotators Training}), each review-summary pair is annotated by a single annotator.
To ensure quality, submissions are randomly sampled and reviewed, with feedback provided as necessary.

\subsection{Guidelines}\label{subsec:guidelines}
We instruct our workers to process the text systematically and align characteristics from each summary sentence to the corresponding spans in the review. 

\paragraph{Summary-related Guidelines}
Annotators receive instructions to separate summary sentences into the distinct characteristics they describe, focusing on various attributes like rooms and staff, and different facets of the same attribute, for instance, room cleanliness versus style.
The complete set of summary-related guidelines is detailed in Appendix~\ref{subsec:Summary-related Guidelines}.

\paragraph{Review-related Guidelines}
Upon identifying a characteristic in the summary, annotators are tasked with locating corresponding spans in the review.
These spans are defined as the minimal spans that adequately express the same information as the summary characteristic, where omitting any content would lose some aspect of that characteristic.
Beyond explicit mentions, our guidelines also encompass two additional alignment variants, as outlined in \S\ref{sec:task_definition}.  Firstly, to accommodate instances where summaries include generalized mentions of highlights, annotators are directed to also identify more specific review excerpts that correspond to the summary characteristic. Secondly, for aggregated abstractions, workers are also instructed to include review spans that exemplify the summary characteristic, such as aligning a review statement like \textit{``the bed was clean''} with a summary phrase \textit{``the rooms are clean''}.
Moreover, given that reviews may express varying opinions about the same feature, annotators are also trained to align review mentions that either match or contradict the sentiment of the summary characteristic. For example, alignments for ``the staff was helpful'' should include both positive and negative mentions of staff helpfulness.
Finally, annotators may mark multiple spans in reviews that redundantly represent the same fact.
The guidelines also address paraphrasing, non-consecutive highlights, and un-alignable summary spans. A detailed explanation of these guidelines could be found in Appendix~\ref{subsec:Review-related Guidelines}.

\subsection{Annotator Training}\label{subsec:Annotators Training}
Employing the Controlled Crowdsourcing methodology \cite{roit-etal-2020-controlled}, we identify qualified annotators through three open qualification rounds, followed by closed rounds for selected annotators, focusing on further training and refinement.
Each round involves annotators reading a brief task description and completing a trial annotation. The closed rounds start with a 25-minute tutorial on the annotation tool and guidelines (see \S\ref{subsec:Annotation Process}).
Each round is thoroughly evaluated by the authors for feedback purposes. 
These qualification rounds are fully compensated, requiring up to 5 minutes to complete, and include 3 summary-review pairs and feedback review. Ultimately, 7 out of 10 initial annotators successfully completed the training.

\paragraph{Cost}
Each annotation instance, averaging 4 minutes, is priced at 70\textcentoldstyle. 
Annotators also receive compensation for training activities, including a 5$\$$ bonus for taking the 25-minute tutorial and an additional 2$\$$ for reviewing feedback. The total cost for the dataset amounted to approximately 5700$\$$.

==> sections/deprecated/6_experimental_setup_deprecated.tex <==
\input{tables/results}
\section{Experimental Setup}\label{sec:experimental_setup}

We examine several baseline models for solving the \fic{} task. The input to a model is a document set with spans marked within the documents (highlights), and the model ouputs a fused passage around the highlights.

\paragraph{Models with full input.}
Using the training set of our dataset, we finetune a large language model, marking the highlights in the input via designated mark-ups, following \citet{slobodkin-etal-2022-controlled}. Specifically, we finetune a \texttt{flan-t5-large} model \citep{https://doi.org/10.48550/arxiv.2210.11416}, that exhibited enhanced performance in tasks requiring constrained generation \citep{sanh2022multitask, wei2022finetuned, zhou2023controlled}. We will refer to this model as \textbf{Flan-T5\textsubscript{H}} (`H' for `Highlights').
We develop an additional variant of Flan-T5\textsubscript{H}, which we further finetune using Reinforcement Learning (\textbf{RL}), following the method in \citet{slobodkin2023dont}. It applies the Quark algorithm \citep{lu2022quark} combined with a dual-reward policy \citep{pasunuru-bansal-2018-multi}, alternating between our NLI-based faithfulness and trained coverage metrics (\S\ref{sec:evaluation_framework}) as rewards.
We also examine the performance of a one-shot \textbf{GPT-4} model \citep{openai2023gpt4}, guided with an example of the task.\footnote{Preliminary experiments on a separate development set, with varying numbers of in-context examples, indicated that a single exemplar yields the best results. See Appendix~\ref{sec:gpt4_prompting}.}
%Utilizing the crowdsourced training dataset, we finetune \texttt{flan-t5-large} \citep{https://doi.org/10.48550/arxiv.2210.11416}, motivated by recent work suggesting enhanced performance of instruction-finetuned models in tasks requiring constrained generation \citep{sanh2022multitask, wei2022finetuned, zhou2023controlled}. Following \citep{slobodkin-etal-2022-controlled}, highlights are marked in the input via designated mark-ups, placed before and after each highlighted span. We will refer to this model as Flan-T5\textsubscript{H}, where 'H' stands for 'Highlights'. 
%An additional variant of Flan-T5\textsubscript{H} is developed, following additional Reinforcement Learning (RL) finetuning, akin to the approach in \citep{slobodkin2023dont}.
%This involves using the Quark algorithm \citep{lu2022quark} combined with a dual-reward policy \citep{pasunuru-bansal-2018-multi}, alternating between our proposed coverage and faithfulness metrics (\S\ref{sec:evaluation_framework}) as rewards.
%Furthermore, we also examine the performance of a single-shot GPT-4 model \citep{openai2023gpt4} when guided with an example of the task.\footnote{Preliminary experiments on a separate development set, with varying numbers of in-context examples, indicated that a single exemplar yields the best results. See Appendix~\ref{sec:gpt4_prompting} for further details.}


\paragraph{Models with highlights only.}
To reveal the importance of the surrounding context, we also train a \texttt{flan-t5-large} model only with a concatenation of the highlights as the input (excluding surrounding context). We denote this variant \textbf{Flan-T5\textsubscript{only-H}}.
%To show the necessity of the surrounding context, we also train a variant of \texttt{flan-t5-large}, where the input consists exclusively of a concatenation of the highlights, excluding any additional surrounding context. we denote this variant Flan-T5\textsubscript{only-H}.

\paragraph{Models without highlights.}
Finally, we examine \texttt{flan-t5-large} in a standard summarization setting, where it is simply finetuned with the input review-set without the highlighted spans. This version is referred to as \textbf{Flan-T5\textsubscript{no-H}}. It offers insights into the model's ability to pick up on signals that point to the highlights.
%We also examine \texttt{flan-t5-large} in a standard summarization setting without highlights, where it is finetuned and evaluated using the original reviews without any highlighted segments. 
%This version is referred to as Flan-T5\textsubscript{NH}, with 'NH' signifying 'No Highlights'.
%This variant aligns with the traditional summarization framework and offers valuable insights into the model's capacity to to pick up the highlighting signals.


% \paragraph{Evaluation}
% Alongside the assessment of highlights coverage and faithfulness, as outlined in Section~\ref{sec:evaluation_framework}, we also adopt the coherency analysis methodology as described by \citep{slobodkin-etal-2022-controlled}. This involves employing crowdworkers to assess the coherency of 100 randomly selected samples from each examined model. The evaluation employs a 5-point Likert scale, and each model's output being reviewed by three separate crowdworkers. Additionally, the redundancy of each model's output is also subjected to a similar evaluation.
% This approach follows the standard common practice, where fluency, coherence, and redundancy are best evaluated manually.
% For more details see Appendix~\ref{sec:Fluency_and_Reduancy_Human_Annotation_Protocol}.


==> sections/deprecated/7_results_deprecated.tex <==
\section{Results}\label{sec:results}

\os{Maybe we can have Section 6 as "Experiments" with current 6 and 7 as subsections.}
We applied our evaluation metrics on the proposed systems, with results presented in \autoref{tab:results}. We first observe that the exclusion of context from the input (Flan-T5\textsubscript{only-H}) yields the strongest faithfulness and coverage scores, however the coherence and redundancy are hindered. This demonstrates the significance of incorporating context for more seamless outputs. Meanwhile, the removal of highlights (Flan-T5\textsubscript{no-H}) results in a substantial degradation in faithfulness and coverage. This indicates that the model does in fact succeed in learning to adjust the output according to the highlights, underlining the highlights' role in enhancing the model's performance.

Interestingly, even though the RL reward functions used in the RL-enriched model are the faithfulness and coverage metrics themselves, the outputs are eventually negatively affected when evaluating with these metrics \os{do we have an intuition for why?}. This result calls for a more thorough investigation, and enhanced reward functions that can leverage the benefits of RL-enrichment, as was shown to be advantageous in \citet{slobodkin2023dont} for the single document setup. Additionally, we find that single-shot GPT-4 yields the most coherent and least redundant texts. While it ranks highly in faithfulness and coverage, it is still overtaken by the fine-tuned Flan-T5\textsubscript{only-H}. Overall, our findings invite for further research on the \fic{} task, to develop fusion strategies that ensure comprehensive coverage and faithfulness to highlighted content, with coherent and low-redundancy outputs.

% \autoref{tab:results} shows the results on our evaluation frameworks. We first observe that the exclusion of context from the input (Flan-T5\textsubscript{only-H}), while enhancing faithfulness and coverage scores, also degrades the quality of outputs in terms of coherence and redundancy. This demonstrates the significance of incorporating context for more fluent outputs. Additionally, the removal of highlights (Flan-T5\textsubscript{no-H}) results in a substantial decline of approximately 20 and 10 points in faithfulness and coverage scores, respectively.
% This indicates that highlights are crucial in guiding the model's focus towards specific, targeted content.

% Interestingly, applying the RL approach from \citep{slobodkin2023dont} with our faithfulness and coverage metrics as rewards seems to negatively impact both metrics. This indicates a need for more innovative scoring methods that can more effectively leverage RL strategies to enhance these metrics. 
% Additionally, we find that GPT-4, when prompted in a single-shot setting, yields the most coherent and least redundant texts. It also ranks highly in faithfulness and coverage. However, we find that the finetuned Flan-T5\textsubscript{H} model exhibits superior coverage compared to GPT-4, pointing to areas where GPT-4 could be further improved. On the other hand, in addition to being substantially less faithful than GPT-4, the finetuned Flan-T5\textsubscript{H} also tends to produce outputs that are less coherent and more redundant. This indicates a need for additional research into fusion strategies that not only ensure comprehensive coverage and faithfulness to highlighted content but also integrate it more coherently and with less repetitions.

